Large Language Models Can Self-Improve in Long-context Reasoning

Large language models (LLMs) have achieved substantial progress in processing long contexts but still struggle with long-context reasoning. Existing approaches typically involve fine-tuning LLMs with synthetic data, which depends on annotations from human experts or advanced models like GPT-4, thus restricting further advancements. To address this issue, we investigate the potential for LLMs to self-improve in long-context reasoning and propose \ours, an approach specifically designed for this purpose. This approach is straightforward: we sample multiple outputs for each question, score them with Minimum Bayes Risk, and then apply supervised fine-tuning or preference optimization based on these outputs. Extensive experiments on several leading LLMs demonstrate the effectiveness of \ours, with an absolute improvement of $4.2$ points for Llama-3.1-8B-Instruct. Furthermore, \ours achieves superior performance compared to prior approaches that depend on data produced by human experts or advanced models. We anticipate that this work will open new avenues for self-improvement techniques in long-context scenarios, which are essential for the continual advancement of LLMs.

==> tables/analysis_of_hallucination.tex <==

\begin{table*}[htbp]
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
    Model                                                             & Long-context Avg.              & Natural Questions             & TriviaQA              & TruthfulQA   \\ 
    \midrule
    Llama-3.1-8B-Instruct \citep{dubey2024llama}                                            & 50.8                           & 30.0                          & 70.2                  & 54.1  \\
    \midrule
    \multicolumn{5}{c}{\textit{Supervised Fine-tuning}} \\          
    \midrule
    \quad + LongReward-SFT \citep{zhao2024wildchat}                     & 47.4                           & 29.8                          & 70.4                  & 53.8 \\
    \quad + GPT-4o \citep{hurst2024gpt}                                 & 50.9                           & 30.0                          & 70.1                  & 54.7 \\
    \quad + \ours-SFT                                                         & 52.4                           & 29.4                          & 70.1                  & 53.7 \\
    \midrule
    \multicolumn{5}{c}{\textit{Preference Optimization}} \\
    \midrule
    \quad + LongReward-Preference \citep{zhang2024longreward}           & 50.9                           & 29.6                          & 70.8                  & 54.1 \\
    \quad + \ours                                                             & 55.0                           & 29.4                          & 70.2                  & 53.8 \\
\bottomrule
\end{tabular}
}
\caption{
Average performance on long-context tasks (Tab. \ref{tab:main_results_datasets}) and factual accuracy in Natural Questions \citep{kwiatkowski2019natural}, TriviaQA \citep{joshi2017triviaqa}, and TruthfulQA \citep{lin2022truthfulqa}. This empirical study explores whether fine-tuning with self-supervision mitigates hallucination risk, specifically in terms of factuality. However, we did not observe a notable difference in hallucination tendencies after fine-tuning on various datasets.
}
\label{tab:hallucination}
\end{table*}

==> tables/iterative_training.tex <==
\begin{table}[htbp]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
    Method                              & HotpotQA           & MuSiQue           & 2WikiMQA           \\ 
    \midrule
    Direct 32K \\
    \midrule
    \multicolumn{4}{c}{\textit{Iterative Training}} \\
    \midrule
    Iteration-1 32K \\
    \quad + Iteration-2 32K \\
    \quad \quad + Iteration-3 32K \\
    \midrule
    Iteration-1 16K \\
    \quad + Iteration-2 24K \\
    \quad \quad + Iteration-3 32K \\
\bottomrule
\end{tabular}
}
\caption{
Comparison of \ours with direct training and iterative training.
}
\end{table}

==> tables/synthesizing_questions.tex <==
\begin{table}[htbp]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
    \textbf{Method}                              & HotpotQA           & MuSiQue           & 2WikiMQA           \\ 
    \midrule
    Random Chunk \\
    \quad \quad $+$ Merge \\
    Entire Context \\
    \quad \quad $+$ Few-shot \\
    \ours   \\
\bottomrule
\end{tabular}
}
\caption{
Comparison of different approaches for synthesizing questions. The metric is SubEM.
}
\end{table}

==> tables/training_strategy.tex <==

\begin{table}[htbp]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
    Training Strategy                         & Long-context Avg.   & Short-context Avg.   \\ 
    \midrule
    Full Parameter                            & 85.3               & 90.7                 \\
    QLoRA \citep{dettmers2024qlora}           & 83.5               & 88.2                 \\
\bottomrule
\end{tabular}
}
\caption{
Comparison of training strategies for long-context and short-context performance, measured on Llama-3.1-Instruct 8B with \ours.
}
\label{tab:training_strategy_comparison}
\end{table}
